Optimal Dynamic Parameterized Subset Sampling

In this paper, we study the Dynamic Parameterized Subset Sampling (DPSS) problem in the Word RAM model. In DPSS, the input is a set,~$S$, of~$n$ items, where each item,~$x$, has a non-negative integer weight,~$w(x)$. Given a pair of query parameters, $(\alpha, \beta)$, each of which is a non-negative rational number, a parameterized subset sampling query on~$S$ seeks to return a subset $T \subseteq S$ such that each item $x \in S$ is selected in~$T$, independently, with probability $p_x(\alpha, \beta) = \min \left\{\frac{w(x)}{\alpha \sum_{x\in S} w(x)+\beta}, 1 \right\}$. More specifically, the DPSS problem is defined in a dynamic setting, where the item set,~$S$, can be updated with insertions of new items or deletions of existing items. Our first main result is an optimal algorithm for solving the DPSS problem, which achieves~$O(n)$ pre-processing time, $O(1+\mu_S(\alpha,\beta))$ expected time for each query parameterized by $(\alpha, \beta)$, given on-the-fly, and $O(1)$ time for each update; here, $\mu_S(\alpha,\beta)$ is the expected size of the query result. At all times, the worst-case space consumption of our algorithm is linear in the current number of items in~$S$. Our second main contribution is a hardness result for the DPSS problem when the item weights are~$O(1)$-word float numbers, rather than integers. Specifically, we reduce Integer Sorting to the deletion-only DPSS problem with float item weights. Our reduction implies that an optimal algorithm for deletion-only DPSS with float item weights (achieving all the same bounds as aforementioned) implies an optimal algorithm for Integer Sorting. The latter remains an important open problem. Last but not least, a key technical ingredient for our first main result is an efficient algorithm for generating Truncated Geometric random variates in $O(1)$ expected time in the Word RAM model.

==> code_nextl.tex <==
\begin{algorithm}
	\caption{PSS algorithm for next-level instances}\label{algo:nextl}
\KwData{A PSS instance $X=\{x_1,\ldots,x_N\}$, the Bucket-Group Structure BG-Str($X$), a PSS query parameter $(\alpha,\beta)$}
\KwResult{The query result $T_{3X}\subseteq X$ of the next-level instance}
Initialize $T_{3X}\leftarrow \emptyset$; $h_1\leftarrow \lfloor \frac{\log_2 {\frac{W}{N^2}}}{\lceil \log_2 N \rceil} -1 \rfloor$; $h_2\leftarrow \lceil \frac{\log W}{\lceil \log N \rceil } \rceil$ \;
\For{$j\in [h_1+1,h_2-1]$, if $G_X(j)$ is non-empty}{
Let $T_{Y_j}$ denote the PSS-Query result on $G_X(j)$ with parameter $(0,W_X(\alpha,\beta))$\;
\For{$B_X(i)\in T_{Y_j}$}{
$p\leftarrow \min\{1,\frac{2^{i+1}}{W_X(\alpha,\beta)}\}$\;
\If {$p=1$}{
$T_{3X}\leftarrow T_{3X}\cup\{x\}$ for each $x$ in $B_X(i)$ with $\min\{1,w(x)/W_X(\alpha,\beta)\}$ probability\;
}
\ElseIf {$p|B_X(i)|\geq 1$}{
$k\leftarrow \Geo(p,|B_X(i)|+1)$\;
\While {$k\leq |B_X(i)|$}{
$T_{3X}\leftarrow T_{3X}\cup\{B_X(i)[k]\}$ with $\frac{w(B_X(i)[k])/W_X(\alpha,\beta)}{p}$ probability\;
$k\leftarrow k+\Geo(p,|B_X(i)|+1)$\;
}
}
\ElseIf{$p|B_X(i)|< 1$}{
$q\leftarrow \frac{1-(1-p)^{|B_X(i)|}}{p|B_X(i)|}$\;
\If {$\Ber(q)=1$}{
$k_1\leftarrow \text{TGeo}(p,|B_X(i)|)$\;
$T_{3X}\leftarrow T_{3X}\cup\{B_X(i)[k_1]\}$ with $\frac{w(B_X(i)[k_1])/W_X(\alpha,\beta)}{p}$ probability\;
$k\leftarrow k_1+\Geo(p,|B_X(i)|+1) $\;
\While {$k\leq |B_X(i)|$}{
$T_{3X}\leftarrow T_{3X}\cup\{B_X(i)[k]\}$ with $\frac{w(B_X(i)[k])/W_X(\alpha,\beta)}{p}$ probability\;
$k\leftarrow k+\Geo(p,|B_X(i)|+1)$\;
}
}
}
}
}

\end{algorithm}

==> sortlist.tex <==
\section{Maintain Sorted List on the Word RAM Model}
\label{sec:appendixsort}
In this section, we provide an implementation to achieve Fact~\ref{fact:sorted}. The input is a set $I$ of $n$ integers from the universe $U=\{0,1,\ldots,d-1\}$ and the data structure supports each of the following operations in $O(1)$ worst-case time:
\begin{itemize}
    \item an insertion of a new integer or a deletion of an existing integer to $I$;
    \item finding the predecessor and successor for any integer $q\in U$ in $I$;
\end{itemize}
The data structure includes a bitmap $\mathcal{M}$, a pointer array $\mathcal{P}$, a menu array $\mathcal{Q}$. 

The bitmap $\mathcal{M}$ is a 1 word integer which contains $d$ bits and the $i$-th bit indicates whether the integer $i$ is in $I$. We can invoke bit-wise operations on $\mathcal{M}$ in $O(1)$ time to answer the predecessor and successor non-empty bucket index. For example, given an integer $q\in U$, the following algorithm returns the successor of $q$ in $I$.
\begin{itemize}
    \item $u\leftarrow \mathcal{M}>> q$, which shifts all the lower $q$ bits out;
    \item If $u=0$, report that the successor of $q$ does not exist in $I$;
    \item Otherwise, compute $q'=q+\log_2(u\mathbin \&\neg (u-1))$;
    \item Return $q'$ as the successor of $q$ in $I$.
\end{itemize}


$\mathcal{P}$ is a dynamic array with $n$ terms and each term stores the pointer to an integer in $I$. Therefore, $\mathcal{P}$ requires $O(n)$ words of storage and can be initialized with $O(n)$ time. 
$\mathcal{Q}$ contains $d$ integers and each of the integers is in the range of $[1,n]$. So each integer occupies at most $O(\log n)$ bits of storage and in total $\mathcal{Q}$ takes $O(\log n)$ words. 
At the beginning of the algorithm, $\mathcal{Q}$ is initialized with all $0$ bits so we can initialize $\mathcal{Q}$ with $O(\log n)$ time; and $\mathcal{P}$ is an empty dynamic array. Then for each of the integer $p\in I$, we push back the pointer of $p$ to $\mathcal{P}$ and set the $p$-th term of $\mathcal{Q}$ as the index of the corresponding term in $\mathcal{P}$. Thus, $\mathcal{Q}$ serves as a menu, allowing us to quickly locate the associated position in $\mathcal{P}$. This step can be done in $O(n)$ time.

After initializing the menu array $\mathcal{Q}$ and the pointer array $\mathcal{P}$, we recursively query the successors with the bitmap $\mathcal{M}$ and link the corresponding integers with a sorted linked list.

Now we consider how to maintain this data structure. We first suppose the insertion and deletion does not change the value of $\lceil \log_2 n\rceil$, thus we do not need to rebuild $\mathcal{Q}$ and $\mathcal{P}$.
When we insert a new integer $q$ to $I$, we set the corresponding bit in $\mathcal{M}$ as 1 and tail insert the pointer $q$ to $\mathcal{P}$ and let the the $q$-th term of $\mathcal{Q}$ store the index of $\mathcal{P}$. Then we find the pointer of $q$'s predecessor or successor and insert $q$ to the correct location in the linked list to maintain it to be sorted.
If we delete an existing integer $p$, we can find the pointer to $p$ and remove it from the linked list. Then we maintain the bitmap $\mathcal{M}$ by setting the corresponding bit as $0$. To maintain $\mathcal{P}$ and $\mathcal{Q}$, we first locate the index of the associated term in $\mathcal{P}$, swap it with the term at the end, and then remove the last term from $\mathcal{P}$. When we do the swapping, the term that was swapped also needs to have its reference in $\mathcal{P}$ updated. All of the operations can be done in $O(1)$ time. 

When the size of $I$ doubles or halves, we can rebuild the entire data structure. The rebuilding cost can be charged to those updates, making each update cost $O(1)$ amortized. Here, we can use de-amortization techniques to ensure the complexity becomes $O(1)$ in the worst case.





==> update-algo.tex <==
\subsection{Handling Updates}
\label{sec:updates}
Next, we discuss how to update our HALT structure on the item set~$S$. 
Specifically, each update on~$S$ is either an insertion of a new item~$x$ with weight~$w(x)$ or a deletion of an existing item~$x$ from~$S$. 
For simplicity, we assume that $\frac{1}{2} n_0 \leq n \leq 2n_0$, where~$n$ is the current size of~$|S|$ after the update.

The HALT structure on~$S$ can be maintained as follows.
First, observe that the lookup table in the HALT structure on~$S$ does not need to be updated.
Second, the three-level sampling hierarchy is basically a hierarchy of sorted lists of buckets and groups with length at most~$O(d)$. Each update operation (either insertion or deletion) on these sorted lists can be easily done in~$O(1)$ time in the Word RAM Model. 
The only issue to be careful about is that
each update operation at the previous level in the hierarchy could trigger a {\em weight update} of a next-level item, which would require two update operations to achieve: delete the item first and then insert the item again with the new weight. 
As the hierarchy has only three levels, therefore, there can be in total at most $O(1)$ update operations to the hierarchy. 
Moreover, there is also only $O(1)$ final-level instances would be affected by an update to $S$. 
Their adapters can be updated simply by updating the corresponding bucket sizes in the sub-array $\mathcal{A}[l_1, l_2]$.
Therefore, the overall update time is bounded by $O(1)$ worst-case time.

To handle the case when $n < \frac{1}{2} n_0$ or $n > 2 n_0$,
we adopt the standard global rebuilding trick to re-construct the entire HALT structure on the current item set~$S$ and update $n_0 \leftarrow n$. 
Recall that the HALT structure on~$S$ can be constructed in~$O(n_0)$ time with~$O(n_0)$ space consumption.
As there must be at least~$\Omega(n_0)$ updates to trigger the reconstruction, 
the rebuilding cost can be charged to those updates making each update cost become~$O(1)$ amortized.
Moreover, the space consumption is bounded by~$O(n)$ all the times.

Interestingly, the~$O(1)$ amortized update time can be easily ``de-amortized'' by applying the same technique for the de-amortization for dynamic arrays, just increasing the space consumption by a constant factor. 
Thus, we have the following theorem.
\begin{theorem}
The HALT structure on item set~$S$ can be maintained in~$O(1)$ worst-case time for each update to~$S$. Space consumption is bounded by~$O(n)$ at all times, where~$n$ is the current size of~$S$. 
\end{theorem}




